VRA: Grounding Discrete-Time Joint Acceleration in Voltage-Constrained Actuation

Discrete-time joint acceleration constraints are widely used to enforce position and velocity limits. However, under voltage-constrained electric actuators, kinematically admissible accelerations may be physically unrealizable, exposing a missing execution-level abstraction. We propose Voltage-Realizable Acceleration (VRA), a joint-level acceleration interface that grounds kinematic acceleration in voltage-constrained actuator physics by restricting commanded accelerations to voltage-realizable constraints. Hardware experiments on electric actuators and a wheel-legged quadruped show that VRA removes unrealizable accelerations, restores consistent near-constraint execution, and reduces constraint-induced oscillations.

==> content/supply.tex <==
\newcommand{\RComment}[1]{\hfill{\footnotesize(\emph{#1})}}
\begin{algorithm}[t]
\caption{Proposed EJAC}
\label{alg:vats}
\begin{algorithmic}[1]
\REQUIRE motor state $x_{k-1}=(q_{k-1},\dot q_{k-1})$, raw acceleration command $\ddot{q}^{\mathrm{raw}}_k$, sampled feedback $i_{q,k-1},\mathbf{u}_{k-1}$, motor parameters, joint position bound $q^{\mathrm{max}}$, execution period $\Delta t$, position look-ahead interval $\Delta t_h$
\ENSURE execution consistent $\ddot{q}_k$
\STATE $\omega_{e,k} \leftarrow \dot{q}_{k-1}G_rN_p$ \RComment{Assumption 1}
\STATE $\boldsymbol{u}_{k-1}^{\mathrm{n}} \leftarrow \mathrm{NominalVoltage} (\omega_{e,k-1},i_{q,k-1})$ \RComment{Eq.~\ref{eq:motor_voltage}}

\STATE $\boldsymbol{u}_k^\mathrm{res} \leftarrow  \boldsymbol{u}_{k-1}^{\mathrm{n}} - \boldsymbol{u}_{k-1}$ \RComment{Assumption 2}

% \STATE $[\tau^{\mathrm{lb}}_{\mathrm{tr},k},\tau^{\mathrm{ub}}_{\mathrm{tr},k}] \leftarrow \mathrm{Solve}\ \mathcal{C}_1(\mathbf{u}_k^\mathrm{res},\omega_{e,k-1},i_{q,k-1},\Delta t)$ \RComment{Eq. \eqref{Eq:quadratic}}

\STATE $\mathcal{S}_{\mathrm{st}} \leftarrow \mathrm{Solve}\ \mathcal{C}_\mathrm{st}(\boldsymbol{u}_k^\mathrm{res},\omega_{e,k-1},i_{q,k-1},\Delta t)$ \RComment{Eq.~\ref{Eq:quadratic}}

% \STATE $[\ddot{q}^{\mathrm{lb}}_{\mathrm{st},k},\ddot{q}^{\mathrm{ub}}_{\mathrm{st},k},\tau^{\mathrm{lb}}_{\mathrm{st},k},\tau^{\mathrm{ub}}_{\mathrm{st},k}] \leftarrow \mathrm{Solve}\ \mathcal{C}_2(\mathbf{u}_k^\mathrm{res},\omega_{e,k-1})$ \RComment{Eq. \eqref{Eq:quadratic}}
\STATE $\mathcal{S}_\mathrm{tr} \leftarrow \mathrm{Solve}\ \mathcal{C}_\mathrm{tr}(\boldsymbol{u}_k^\mathrm{res},\omega_{e,k-1}, \Delta t)$ \RComment{Eq.~\ref{Eq:quadratic}}

% \STATE $[\tau^{\mathrm{lb}}_{\mathrm{fi},k},\tau^{\mathrm{ub}}_{\mathrm{fi},k}] \leftarrow [\mathrm{max}(\tau^{\mathrm{lb}}_{\mathrm{tr},k},\tau^{\mathrm{lb}}_{\mathrm{st},k}),\mathrm{min}(\tau^{\mathrm{ub}}_{\mathrm{tr},k},\tau^{\mathrm{ub}}_{\mathrm{st},k})]$
\STATE $\mathcal{S}_{\mathrm{fi}}=\mathcal{S}_{\mathrm{st}} \cap \mathcal{S}_\mathrm{tr}$
\STATE $[\ddot{q}_{\mathrm{fi},k}^{\mathrm{lb}},\ddot{q}_{\mathrm{fi},k}^{\mathrm{ub}}] \leftarrow $ NominalDynamics$(\{\tau_k,\tau_k\in \mathcal{S}_\mathrm{fi}\})$
\STATE $\ddot{q}_k^{\mathrm{max}} \leftarrow \mathrm{SelectDecelerationAuthority}(\dot{q}_{k-1},\ddot{q}^{\mathrm{lb}}_{\mathrm{fi},k},\ddot{q}^{\mathrm{ub}}_{\mathrm{fi},k})$
\STATE $[\ddot{q}^{\mathrm{lb}}_{\mathrm{p},k},\ddot{q}^{\mathrm{ub}}_{\mathrm{p},k}] \leftarrow \mathrm{KinematicEnvelop}(\Delta t_p,q^\mathrm{max}, a_k^{\mathrm{max}})$ 
% \RComment{\cite{PreteVK}}
\STATE $\ddot{q}_{\mathrm{p},k} \leftarrow \mathrm{Clamp}(\ddot{q}^{\mathrm{lb}}_{\mathrm{p},k},\ddot{q}^{\mathrm{ub}}_{\mathrm{p},k},\ddot{q}_k^{\mathrm{raw}})$
\STATE $\ddot{q}_k \leftarrow \mathrm{Clamp}(\ddot{q}^{\mathrm{lb}}_{\mathrm{fi},k},\ddot{q}^{\mathrm{ub}}_{\mathrm{fi},k},\ddot{q}_{\mathrm{p},k})$
\RETURN $\ddot{q}_k$
\end{algorithmic}
\end{algorithm}
